Pretraining in Deep Reinforcement Learning: A Survey

The past few years have seen rapid progress in combining reinforcement learning (RL) with deep learning. Various breakthroughs ranging from games to robotics have spurred the interest in designing sophisticated RL algorithms and systems. However, the prevailing workflow in RL is to learn tabula rasa, which may incur computational inefficiency. This precludes continuous deployment of RL algorithms and potentially excludes researchers without large-scale computing resources. In many other areas of machine learning, the pretraining paradigm has shown to be effective in acquiring transferable knowledge, which can be utilized for a variety of downstream tasks. Recently, we saw a surge of interest in Pretraining for Deep RL with promising results. However, much of the research has been based on different experimental settings. Due to the nature of RL, pretraining in this field is faced with unique challenges and hence requires new design principles. In this survey, we seek to systematically review existing works in pretraining for deep reinforcement learning, provide a taxonomy of these methods, discuss each sub-field, and bring attention to open problems and future directions.

==> alg/offline.tex <==
%% This declares a command \Comment
%% The argument will be surrounded by /* ... */
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}
\SetAlgorithmName{Protocol}{protocol}{List of Protocols}
\caption{Pretraining via Offline Representation Learning}\label{alg:offline}
\KwData{$n \geq 0$}
\KwResult{$y = x^n$}
$y \gets 1$\;
$X \gets x$\;
$N \gets n$\;
\While{$N \neq 0$}{
  \eIf{$N$ is even}{
    $X \gets X \times X$\;
    $N \gets \frac{N}{2}$ \Comment*[r]{This is a comment}
  }{\If{$N$ is odd}{
      $y \gets y \times X$\;
      $N \gets N - 1$\;
    }
  }
}
\end{algorithm}

==> alg/online.tex <==
%% This declares a command \Comment
%% The argument will be surrounded by /* ... */
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}
\SetAlgorithmName{Protocol}{protocol}{List of Protocols}
\caption{Pretraining via Online Exploration}\label{alg:online}
\KwData{$n \geq 0$}
\KwResult{$y = x^n$}
\For{$e=0$ \KwTo $K$}{
    \For{$t=0$ \KwTo $T$}{
       receive observation $o_t$ from environment\;
       take action $a_{t} \sim \pi\left(\cdot \mid o_{t}\right)$\;
       receive observation $o_{t+1}$ and $\bcancel{r_t}$\;
       update buffer $\mathcal{D} \leftarrow \mathcal{D} \cup\left(s_{t}, a_{t}, s_{t}^{\prime}\right)$\;
       sample batch $\left\{\left(s_{i}, a_{i}, s_{i}^{\prime}\right)\right\}_{i=1}^{N} \sim \mathcal{D}$\;
       \For{$i=0$ \KwTo $N$}{
            compute target value $\hat{Q}_{i}=Q_{\theta^{\prime}}\left(s_{i}^{\prime}, a_{i}^{\prime}\right)$, $a_{i}^{\prime} \sim \pi\left(\cdot \mid s_{i}^{\prime}\right)$\;
            compute intrinsic reward $r_i$\;
       }
       compute loss $l = \sum_{i}\left(Q\left(s_{i}, a_{i}\right)-r_i-\hat{Q}_{i}\right)^{2}$\;
       take one gradient step\;
    }
}
\end{algorithm}

==> fig/online_comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/online_comparison.jpg}
    \caption{Do we need this kind of comparison?}
    \label{fig:online_comparison}
\end{figure}

==> sec/6-theoretical.tex <==
\section{Theoretical Results}\label{sec:theory}
\cite{eysenbach2022the} "provide a geometric perspective on these skill learning methods."

\cite{mutti2022importance} "argue that
non-Markovianity is instead paramount for maxi-
mum state entropy exploration in a finite-sample
regime."

"The problem of unsupervised pretraining for RL has also been studied in the RL theory community [2,
39, 40], where it is referred to as the reward-free setting. The algorithms proposed in these prior
works use a version of goal-conditioned RL for pretraining. However, the aim of these methods is
different from ours: these methods aim to collect a sufficient breadth of data, whereas we focus on
learning good representations."~\cite{eysenbach2022the}

\paragraph{Theoretical Results}
"On the theoretical side, questions of representation learning have received an increased recent emphasis owing
to their practical significance, both in supervised learning and RL settings. In RL, a limited form of transfer learning
across multiple downstream reward functions is enabled by several recent reward-free representation learning
approaches (Jin et al., 2020a; Zhang et al., 2020; Wang et al., 2020; Du et al., 2019; Misra et al., 2020; Agarwal et al.,
2020; Modi et al., 2021). Inspired by recent treatments of representation transfer in supervised (Maurer et al., 2016;
Du et al., 2020) and imitation learning (Arora et al., 2020), some works also study more general task collections in
bandits (Hu et al., 2021; Yang et al., 2020, 2022) and RL (Hu et al., 2021; Lu et al., 2021). Almost all these works
study settings where the representation is frozen after pre-training in the source tasks, and a linear policy or optimal
value function approximation is trained in the target task using these learned features. This setting, which we call
representational transfer, is the main focus of our paper"~\shortcite{agarwal2022provable}.

==> sec/proof.tex <==
\section{Proofs}
\subsection{Policy Gradient of discounted state visitation distribution}
Exploration by Maximizing Renyi Entropy for Reward-Free RL Framework: Appendix D.

==> tab/downstream_setup.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
        \thickhline
        & Few-shot & Zero-shot \\
        Same-domain & \cmark & $\star$ & $\star$\\
        Cross-domain & \xmark & $\star\star$ & $\star$\\
        \thickhline
    \end{tabular}
    \caption{Downstream setups.}
    \label{tab:downstream}
\end{table}

==> tab/online.tex <==
\begin{table*}[t]
    \centering
    \scriptsize
    \begin{tabular}{lcccc}
        \thickhline
        \textbf{Algorithm} & \textbf{Component(s)} & \textbf{Objective} & \textbf{Visual} & \textbf{Cross-domain}\\
        \hline
        \multicolumn{5}{l}{\textit{Reward-free pretraining}} \\
        \hline
        CBB~\shortcite{bellemare2016unifying} & $\policy$ & $\max \mathbb{E}_{s}[c(s)]$ & \xmark \\
        DIAYN~\shortcite{eysenbach2018diversity} & $\pi(a \mid s, z)$  & $\max -\mathrm{H}(z \mid s)+\mathrm{H}(a \mid z, s)$ & \xmark\\
        % VIC~\shortcite{gregor2016variational} & \\
        VISR~\shortcite{Hansen2020Fast} & $\psi(s, z), \phi(s)$ & $\max -\mathrm{H}(z \mid s)$ & \cmark\\
        UPSIDE~\shortcite{kamienny2022direct} & $\policy$ & MI & \xmark \\
        MaxEnt~\shortcite{hazan2019provably} & $\pi(a \mid s)$ & $\max H(s)$ & \xmark\\
        CBB~\shortcite{bellemare2016unifying} & $\pi(a \mid s)$ & $\max \mathbb{E}_{s}[c(s)]$ & \xmark\\
        DADS~\shortcite{Sharma2020Dynamics-Aware} & $\pi(a \mid s, z), q\left(s^{\prime} \mid s, z\right)$  & $\max \mathrm{H}(s)-\mathrm{H}(s \mid z)$ & \xmark\\
        EDL~\shortcite{campos2020explore} & $\pi(a \mid s, z)$  & $\max \mathrm{H}(s)-\mathrm{H}(s \mid z)$ & \xmark\\
        APT~\shortcite{liu2021behavior} & $\pi(a \mid s), Q(s, a)$ & $\max H(s)$ & \cmark\\
        APS~\shortcite{liu2021aps} & $\psi(s, z), \phi(s)$ & $\max \mathrm{H}(s)-\mathrm{H}(s \mid z)$ & \cmark \\
        IBOL~\shortcite{kim2021unsupervised} & $\cpolicy$ & $\max \mathbb{E}_{t}\left[I\left(Z ; G_{t} \mid S_{t}\right)-\beta \cdot I\left(Z ; S_{0: T}\right)\right]$ & \xmark \\
        LSD~\shortcite{park2022lipschitzconstrained} & $\cpolicy$ & $\max I(Z ; S)$ & \xmark \\
        Proto-RL~\shortcite{yarats2021reinforcement} & $\encoder$, prototypes & $\max H(s)$ & \cmark \\
        MUSIC~\shortcite{zhao2021mutual} & $\pi(a \mid s)$ & $\max I\left(S^{a} ; S^{S}\right)$ & \xmark \\
        HSD-3~\shortcite{gehring2021hierarchical} & $\pi\left(a \mid s^{p}, F, g\right)$ & distance-based & \xmark & additional objects\\
        ICM~\shortcite{pathak2017curiosity} & $\pi(a \mid s)$ & prediction error & \cmark \\
        % RND~\shortcite{burda2018exploration} & \\
        SMM~\shortcite{lee2019efficient} & $\pi(a \mid s)$ & $\max H(s)$ & \xmark\\
        RE3~\shortcite{seo2021state} & $\pi(a \mid s)$ & $\max H(s)$ & \cmark\\
        % Novelty~\shortcite{tao2020novelty} & \\
        % NGU~\shortcite{Badia2020Never} & & pseudo-count & \cmark \\
        CRL~\shortcite{du2021curious} & $\encoder$ & $\min \mathcal{L}_{\text {contrast}}$ & \cmark\\
        Plan2Explore~\shortcite{sekar2020planning} & World Model & ensemble & \cmark & same domain, multi tasks\\
        HIDIO~\shortcite{zhang2021hierarchical} & \\
        VALOR~\shortcite{achiam2018variational} & \\
        \thickhline
    \end{tabular}
    \caption{
    Classification of the surveyed papers.
    \zhihui{
    Some are borrowed from APT paper.
    Will be updated soon.
    }}
    \label{tab:online}
\end{table*}


==> tab/setting.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
        \thickhline
        \textbf{Setting} & \textbf{Supervision} & \textbf{Task Scalability} & \textbf{Modality Scalability} \\
        \hline
        Naive Pretraining & \cmark & $\star$ & $\star$\\
        Online Pretraining & \xmark & $\star\star$ & $\star$\\
        Offline Pretraining & \xmark & $\star\star$ & $\star$\\
        Generalist Pretraining & \xmark & $\star\star\star$ & $\star\star\star$\\
        \thickhline
    \end{tabular}
    \caption{Comparison between different pretraining settings.}
    \label{tab:setting}
\end{table}
